LOS/NLOS Estimators for mmWave Cellular Systems With Blockages

Designers of millimeter wave (mmWave) cellular systems need to evaluate line-of-sight (LOS) maps to provide good service to users in urban scenarios. In this letter, we derive estimators to obtain LOS maps in scenarios with potential blocking elements. Applying previous stochastic geometry results, we formulate the optimal Bayesian estimator of the LOS map using a limited number of actual measurements at different locations. The computational cost of the optimal estimator is derived and is proven to be exponential in the number of available data points. An approximation is discussed, which brings the computational complexity from exponential to quasi-linear and allows the implementation of a practical estimator. Finally, we compare numerically the optimal estimator and the approximation with other estimators from the literature and also with an original heuristic estimator with good performance and low computational cost. For the comparison, both synthetic layouts and a real layout of Chicago have been used.

==> Sections/preamble.tex <==
%This file contains all the used packages (even more) and definitions and commands.

\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{mathtools}
\usepackage{bbm}
\usepackage{blindtext}
\usepackage[utf8]{inputenc}
\usepackage{float}
\usepackage{enumitem}
\usepackage{hyperref}

\usepackage{graphicx}
\usepackage{subfig}
\usepackage{tikz}
\usetikzlibrary{math}
\usetikzlibrary{calc}

\usepackage{subfig}
\usepackage{siunitx}
\usepackage{url}


\bibliographystyle{IEEEtran}

% Commands and math operators
\newcommand{\prob}[1]{\mathbb{P}(#1)}  % Probability statement
\newcommand{\probc}[2]{\mathbb{P}(#1 \;|\; #2)}  % Conditional Probability
\newcommand{\esp}[1]{\mathbb{E}[#1]}

